Data-Driven Prediction of Route-Level Energy Use for Mixed-Vehicle Transit Fleets

Due to increasing concerns about environmental impact, operating costs, and energy security, public transit agencies are seeking to reduce their fuel use by employing electric vehicles (EVs). However, because of the high upfront cost of EVs, most agencies can afford only mixed fleets of internal-combustion and electric vehicles. Making the best use of these mixed fleets presents a challenge for agencies since optimizing the assignment of vehicles to transit routes, scheduling charging, etc. require accurate predictions of electricity and fuel use. Recent advances in sensor-based technologies, data analytics, and machine learning enable remedying this situation; however, to the best of our knowledge, there exists no framework that would integrate all relevant data into a route-level prediction model for public transit. In this paper, we present a novel framework for the data-driven prediction of route-level energy use for mixed-vehicle transit fleets, which we evaluate using data collected from the bus fleet of CARTA, the public transit authority of Chattanooga, TN. We present a data collection and storage framework, which we use to capture system-level data, including traffic and weather conditions, and high-frequency vehicle-level data, including location traces, fuel or electricity use, etc. We present domain-specific methods and algorithms for integrating and cleansing data from various sources, including street and elevation maps. Finally, we train and evaluate machine learning models, including deep neural networks, decision trees, and linear regression, on our integrated dataset. Our results show that neural networks provide accurate estimates, while other models can help us discover relations between energy use and factors such as road and weather conditions.

==> tables/symbols.tex <==
\begin{table}[h!]
\centering
\caption{List of Symbols}
\label{tab:Symbols}
\begin{tabular}{|c||c|}
\hline
\textbf{Symbols}& \textbf{Description} \\
\hline
\hline $A$ & Battery current [A]\\
\hline $V$ & Battery voltage [V]\\
\hline $P$ & Power [W]\\
\hline $TS$ & Timestamp\\
\hline $SoC$ & State of Charge [\%]\\
\hline $G$ & Geometry string with all the coordinates\\
& for a particular OSM road segment \\
\hline $loc_0$ & Initial GPS location recorded by ViriCiti\\
\hline $loc_n$ & Final GPS location recorded by ViriCiti\\
\hline $L$ & Length of line segment\\
\hline $index_{S}$ & Index of Start Line\\
\hline $index_{E}$ & Index of End Line\\
\hline

\end{tabular}
\end{table}
